APE: Faster and Longer Context-Augmented Generation via Adaptive Parallel Encoding

Context-augmented generation (CAG) techniques, including RAG and ICL, require the efficient combination of multiple contexts to generate responses to user queries. Directly inputting these contexts as a sequence introduces a considerable computational burden by re-encoding the combined selection of contexts for every request. To address this, we explore the promising potential of parallel encoding to independently pre-compute and cache each context's KV states. This approach enables the direct loading of cached states during inference while accommodating more contexts through position reuse across contexts. However, due to misalignments in attention distribution, directly applying parallel encoding results in a significant performance drop. To enable effective and efficient CAG, we propose Adaptive Parallel Encoding ($\textbf{APE}$), which brings shared prefix, attention temperature, and scaling factor to align the distribution of parallel encoding with sequential encoding. Results on RAG and ICL tasks demonstrate that APE can preserve 98% and 93% sequential encoding performance using the same inputs while outperforming parallel encoding by 3.6% and 7.9%, respectively. It also scales to many-shot CAG, effectively encoding hundreds of contexts in parallel. Efficiency evaluation shows that APE can achieve an end-to-end 4.5$\times$ speedup by reducing 28$\times$ prefilling time for a 128K-length context.

==> tables/efficiency.tex <==
\begin{table}[b]
\centering
\caption{Latency on H100 GPU: [prefill / total time (ms)]. The gray text in brackets is batch size.}
\resizebox{\linewidth}{!}{\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|rrrrrrr}
\toprule
Methods & 4K& 8K& 16K & 32K & 64K & 128K \\ \midrule
Sequential Encoding \color{gray}{(1)} & 132/2383 & 276/2558 & 635/3204 & 1646/4713 & 4892/8804 & 16635/22252 \\
MInference \color{gray}{(1)} & 964/3221 & 1297/3609 & 1623/4201 & 2206/5274 & 3563/7458 & 6457/12085 \\
\rowcolor{cyan!10}APE \color{gray}{(1)} & 28/2279 & 40/2322 & 68/2637 & 122/3189 & 226/4138 & 421/6038 \\
\midrule
Sequential Encoding \color{gray}{(4)} & 523/3129 & 1084/4179 & 2558/6474 & 6599/12055 & 19468/28367 & 65928/83869 \\
MInference \color{gray}{(4)} & 3789/6373 & 4995/8099 & 6300/10244 & 8470/13944 & 13462/22313 & 24199/42013\\
\rowcolor{cyan!10}APE \color{gray}{(4)} & 69/2675 & 94/3189 & 150/4066 & 298/5754 & 430/9329 & 858/18799 \\
  \bottomrule
\end{tabular}}}
\label{tab:efficieny}
\end{table}

==> tables/ruler.tex <==
\begin{table}[t]
\centering
\caption{Performance of different models and different methods on RULER \citep{hsieh2024ruler} evaluated at length of 128K. \Sys outperforms other methods with a 1.56\% sparse budget. }
%\renewcommand{\arraystretch}{0.8} % 调整行间距
\setlength{\tabcolsep}{3.1pt} % 调整列间距
\footnotesize
\begin{tabular}{l|rrrrrrrrrr|r}
\toprule
Methods &  N-S1 & N-S2 & N-MK1&N-MK2&N-MQ&N-MV&QA-1&QA-2&VT&FWE &Avg.\\ \midrule
	\textit{Llama-3-8B-1M} & 100.00&100.00&98.96&98.96&98.96&95.57&75.00&48.96&78.54&71.85 & 86.68\\
    Loki & 18.75 & 1.04 & 2.08 & 0.00 & 1.56 & 0.78 & 4.17 & 13.54 & 26.04 & 25.35 & 9.33\\
    Loki (V only) & 41.67 & 6.25 & 37.50 & 1.04 & 8.07 & 30.73 & 10.42 & 19.79 & 51.67 & 37.50& 24.46 \\
    
    \textcolor{blue}{InfiniGen} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{98.96} & \textcolor{blue}{84.38} & \textcolor{blue}{53.13} & \textcolor{blue}{63.28} & \textcolor{blue}{54.95} & \textcolor{blue}{65.63} & \textcolor{blue}{48.96} & \textcolor{blue}{\textbf{81.67}} & \textcolor{blue}{50.35} & \textcolor{blue}{70.13} \\
    \textcolor{blue}{InfiniGen (V only)} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{98.96} & \textcolor{blue}{96.88} & \textcolor{blue}{76.04} & \textcolor{blue}{81.25} & \textcolor{blue}{77.08} & \textcolor{blue}{67.71} & \textcolor{blue}{50.00} & \textcolor{blue}{\textbf{81.67}} & \textcolor{blue}{53.47} & \textcolor{blue}{78.31} \\
    
    Quest & \textbf{100.00} & \textbf{100.00}& \textbf{98.96} & 77.08 & 97.65 & 93.49 & 60.42 & 50.00 & 77.08 & 65.63 & 82.03  \\
    Quest (V only) & \textbf{100.00} & \textbf{100.00} &\textbf{98.96} & 85.42 & \textbf{97.92} & 95.49 & 70.83 & 46.88 & 78.75 & 65.63&83.99\\
	\rowcolor{cyan!10}
	\Sys  & \textbf{100.00} & \textbf{100.00} & 97.92&\textbf{98.96}&96.88&\textbf{95.83}&\textbf{72.92}&\textbf{52.08}&\textbf{81.67}&\textbf{72.57}&\textbf{86.88}\\
	
    \midrule
    \textit{GLM-4-9B-1M}&100.00 & 100.00 & 94.79&87.50&99.74&93.75&67.71&55.21&97.29&72.22&86.82 \\
    
    Loki & 71.88 & 27.08 & 22.92 & 2.08 & 9.90 & 11.46 & 28.13 & 27.08 & 31.04 & 54.17& 28.57\\
    Loki (V only) & 96.88 & 55.21 & 56.25 & 18.75 & 51.04 & 50.52 & 45.83 & 39.58 & 72.71 & 59.72 & 54.65\\
    
    \textcolor{blue}{InfiniGen} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{93.75} & \textcolor{blue}{82.29} & \textcolor{blue}{0.00} & \textcolor{blue}{79.43} & \textcolor{blue}{60.16} & \textcolor{blue}{57.29} & \textcolor{blue}{53.13} & \textcolor{blue}{92.71} & \textcolor{blue}{57.29} & \textcolor{blue}{67.60} \\
    \textcolor{blue}{InfiniGen (V only)} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{96.88} & \textcolor{blue}{87.50} & \textcolor{blue}{7.29} & \textcolor{blue}{95.31} & \textcolor{blue}{75.26} & \textcolor{blue}{56.25} & \textcolor{blue}{54.17} & \textcolor{blue}{95.63} & \textcolor{blue}{60.76} & \textcolor{blue}{72.91} \\
    
    Quest &  \textbf{100.00} & 95.83 & 90.62 & 54.17 & 94.01 & 76.30 & 55.21 & 52.08 & 95.83 & 64.58 & 77.86 \\
    Quest (V only) &  \textbf{100.00} & 96.88 & 93.75 & 72.92 & 95.83 & 83.07 & 56.25 & 53.13 & 96.88 & 65.97 & 81.47\\
    \rowcolor{cyan!10}
    \Sys  & \textbf{100.00}&\textbf{100.00}&\textbf{95.83}&\textbf{83.33}&\textbf{98.70}&\textbf{87.76}&\textbf{69.79}&\textbf{55.21}&\textbf{97.50}&\textbf{68.06}&\textbf{85.62}\\

\midrule
\textit{Llama-3.1-8B} & 100.00 & 100.00 & 98.96 & 91.67 & 98.96 & 95.31 & 82.29 & 47.92 & 68.96 & 71.18 &85.53\\
Loki & 68.75 & 32.29 & 32.29 & 20.83 & 42.71 & 28.65 & 41.67 & 33.33 & 24.79 & 29.86&35.52\\
Loki (V only) & 95.83 & 36.46 & 57.29 & 62.50 & 77.86 & 70.83 & 69.79 & 39.58 & 35.21 & 37.50&58.29\\

\textcolor{blue}{InfiniGen} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{77.08} & \textcolor{blue}{78.13} & \textcolor{blue}{13.54} & \textcolor{blue}{58.07} & \textcolor{blue}{47.40} & \textcolor{blue}{65.63} & \textcolor{blue}{41.67} & \textcolor{blue}{60.83} & \textcolor{blue}{50.35} & \textcolor{blue}{59.27} \\
\textcolor{blue}{InfiniGen (V only)} & \textcolor{blue}{\textbf{100.00}} & \textcolor{blue}{88.54} & \textcolor{blue}{87.50} & \textcolor{blue}{26.04} & \textcolor{blue}{79.43} & \textcolor{blue}{77.08} & \textcolor{blue}{72.92} & \textcolor{blue}{43.75} & \textcolor{blue}{57.08} & \textcolor{blue}{55.21} & \textcolor{blue}{68.76} \\

Quest &  \textbf{100.00} & 98.96 & 97.92 & 34.38 & 93.49 & 88.54 & 70.83 & 44.79 & 65.63 & \textbf{68.40} & 76.29  \\
Quest (V only) & \textbf{100.00} & 98.96 & 98.96 & 56.25 & 95.83 & 90.63 & 76.04 & 46.88 & 66.25 & 67.36&79.72\\

\rowcolor{cyan!10}
\Sys  & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{83.33} & \textbf{97.92} & \textbf{92.19} & \textbf{81.25} & \textbf{48.96} & \textbf{67.08} & 64.93 &\textbf{83.57}\\

 %     \midrule
 %        \textit{Yi-9B-200K}& 100.00& 100.00 & 86.46&62.50&64.58&32.55&44.79&39.58&36.87&89.93 & 65.73\\
 %         Loki & 34.38 & 2.08& 2.08 & 0.00 & 0.00 & 0.52 & 22.92 & 21.88 & 0.00 & 25.00& 10.89\\
 %         Loki (V only) & 59.38 & 11.46 & 18.75 & 5.21 & 4.43 & 2.08 & 22.92 & 31.25 & 0.00 & 35.07 & 19.06\\
	% Quest &  \textbf{100.00} & 98.96 & 79.17 & 26.04 & 56.51& 31.77 & 32.29 & 31.25 & 51.04 & 71.88 &57.89\\
 %         Quest (V only) &\textbf{100.00} & \textbf{100.00} & 80.21 & 45.83 & 59.37 & \textbf{31.90} & 36.45 & 34.37 & 53.54 & 71.88 & 61.36\\
	% \rowcolor{cyan!10}
	% \Sys  & \textbf{100.00} & \textbf{100.00} & \textbf{82.29} & \textbf{67.71} & \textbf{63.28} & 31.51 & \textbf{43.75}&\textbf{38.54} & \textbf{56.04}&\textbf{72.22}&\textbf{65.53}\\

  \bottomrule
\end{tabular}
\label{tab:ruler}
\end{table}
